TPMDP: Threshold Personalized Multi-party Differential Privacy via Optimal Gaussian Mechanism

In modern distributed computing applications, such as federated learning and AIoT systems, protecting privacy is crucial to prevent adversarial parties from colluding to steal others' private information. However, guaranteeing the utility of computation outcomes while protecting all parties' data privacy can be challenging, particularly when the parties' privacy requirements are highly heterogeneous. In this paper, we propose a novel privacy framework for multi-party computation called Threshold Personalized Multi-party Differential Privacy (TPMDP), which addresses a limited number of semi-honest colluding adversaries. Our framework enables each party to have a personalized privacy budget. We design a multi-party Gaussian mechanism that is easy to implement and satisfies TPMDP, wherein each party perturbs the computation outcome in a secure multi-party computation protocol using Gaussian noise. To optimize the utility of the mechanism, we cast the utility loss minimization problem into a linear programming (LP) problem. We exploit the specific structure of this LP problem to compute the optimal solution after O(n) computations, where n is the number of parties, while a generic solver may require exponentially many computations. Extensive experiments demonstrate the benefits of our approach in terms of low utility loss and high efficiency compared to existing private mechanisms that do not consider personalized privacy requirements or collusion thresholds.

==> discussion.tex <==
%In this section, we discuss generalizations of our formulation and the proposed mechanism, as well as the algorithm for statistically and computationally TPMDP multi-party Gaussian mechanisms.

%First, as mentioned in Section \ref{sec:prob}, the results given for $x_i\in \{0, 1\}^*,\, i\in \{1,\hdots,n\}$ can also be generalized to the case where $x_i\in (\{0, 1\}^*)^{\left |x_i \right |},\, i\in \{1,\hdots,n\}$. The second topic is about the generalization of multi-party Gaussian mechanism, in which we would also leave an open problem.


\textbf{Generalization of TPMDP when each party holds multiple inputs.} 
%Consider the definition of TPMDP in case each party holds multiple inputs, i.e., $x_i\in (\{0, 1\}^*)^{l_i},\, i\in \{1,\hdots,n\}$. 
%The definition for TPMDP where each party holds multiple inputs can be derived from Definition \ref{def:tMDP} 
\comment{TPMDP with multiple inputs uses a neighboring relation where a single party's inputs differ by just one. }Formally, Definition \ref{def:tMDP} can be extended to handle the case where each party holds multiple inputs
by varying the domain of $x_i$, i.e., $\{0,1\}^*$ to $x_i\in (\{0, 1\}^*)^{l_i}$ for $i\in \{1,\hdots,n\}$, where $l_i$ stands for the number of inputs party $u_i$ holds.
%cf. Definition \ref{def:tMDP} is based on the refined view (cf. Definition \ref{def:rView}), $j$-neighboring inputs (cf. Definition \ref{def:A_neigh_in}) and $A$-i.i.d randomness (cf. Definition \ref{def:A_iid}). 
%One can verify that Definition \ref{def:rView}, Definition \ref{def:A_neigh_in} and Definition \ref{def:A_iid} can be directly generalized to the case where $x_i\in (\{0, 1\}^*)^{l_i},\, i\in \{1,\hdots,n\}$. 
%Thus Definition \ref{def:rView} can be generalized to the case each party holding multiple inputs. 
All results in Sections \ref{sec:prob} and \ref{sec:res} 
%and \ref{sec:comp} 
hold for this generalized case.

\textbf{Multi-party Gaussian mechanism for general query functions.} 
%Multi-party Gaussian mechanism can be generalized to the case where the query function $f(\cdot)$ is in the general form, i.e., $f_i(\cdot),\, i\in \{1,\hdots,n\}$ can be arbitrarily different functions. 
%The main difference from the query functions we considered in Section \ref{sec:prob} is that the partial $l_2$ sensitivity (cf. \ref{def:p_l2_sensitivity}) is totally different in this case. Notice that for the query functions we considered in Section \ref{sec:prob}, the output observed by $A\in \mathcal{A}_\tau$ can only be either $F(\cdot)$ or $\perp$ while for the general query functions, the output for $A\in \mathcal{A}_\tau$ can be totally different. 
\comment{For multi-party Gaussian mechanisms with general query functions where the outputs revealed to parties are different, there are exponentially many possibilities for leakage, hence the sensitivity computations become more complicated ($n$ choose $\tau$). }Formally, denote the non-repeating functions in $f_i(\cdot),\, i\in \{1,\hdots,n\}$ by $F_i(\cdot),\, i\in \{1,\hdots,m\}$, i.e., $\{f_i(\cdot)\}_{i=1}^n = \{F_i(\cdot)\}_{i=1}^m$ and $F_i(\cdot)\neq F_j(\cdot)$ for $i\neq j$. Let the map $h: 2^{\{1,\hdots,n\}}\rightarrow 2^{\{1,\hdots,m\}}$ satisfy $\{f_i(\cdot)\}_{i\in E} = \{F_i(\cdot)\}_{i\in h(E)}$ for $E\subset \{1,\hdots,n\}$ and the output of the general query function for $A\in \mathcal{A}_\tau$ be $F^{(A)} = (F_i(\cdot))_{i\in h(A)}$. 
One can verify that the results in Section \ref{sec:prob} hold for this case by replacing $F$ with $F^{(A)}$. 
However, results in Section \ref{sec:res} are not immediate to extend for the general query function since in this case the partial $l_2$-sensitivity $\Delta_{2,j} F^{(A)}$ depends not only on $j$ but also on $A$ for $j\in A$ and $A\in \mathcal{A}_\tau$, which implies that the constraint set in Eq.~\eqref{eq:Gauss_opt} becomes much more complicated. We plan to investigate an efficient algorithm for this case in future.

\hide{
\textbf{Applicability to real-world scenarios.} 
%Our proposed mechanism can be applied to design some real-world applications in privacy preserving multi-party collaborative computation. 
Our proposed mechanism can be adopted to design various distributed privacy-preserving machine learning systems such as collaborative filtering, linear regression, and deep learning.
Note that the multi-party Gaussian mechanism is independent of the underlying MPC protocols when the MPC protocol satisfies Theorem \ref{thm:DP_multi_Gaussian_perf} (or Theorem \ref{thm:DP_multi_Gaussian_stat}, Theorem \ref{thm:DP_multi_Gaussian_comp}). 
This property of our design is especially useful since some MPC protocols can be particularly efficient for specific applications.
}

{\textbf{TPMDP mechanisms beyond Gaussian.} 
\comment{For non-Gaussian noise, which generally cannot be constructed by simply adding several components, one may generate it from a random seed collaboratively generated by all parties (e.g. via inverse transform to sample from the noise CDF). This design is indeed a distributed simulation of the \emph{MIN} baseline, the centralized mechanism where there exists a trusted party. However, these operations are highly non-linear (e.g., inverse transform for general noise CDF), while the basic components of arithmetic MPC enlist secure addition and multiplication. Thus, TPMDP mechanisms with general additive noise can be expensive in communication. We leave the details of an efficient construction of TPMDP mechanism for general noise as future work.
As a special case, it is possible to construct Laplace noise from $\mathcal{O}(1)$ Gaussian noise terms~\cite{goryczka2013secure}, in which case it is possible to add personalized Laplace noise in the TPMDP setting with $\mathcal{O}(n)$ communication overhead. We plan to investigate how to design $(\tau, n, ((\epsilon_i, 0))_{i\in U})$-TPMDP mechanisms via the Laplace mechanism in our future work.}
}

{
\textbf{Comparison with LDP and PDP mechanisms.} The focus of this paper is to evaluate the utility loss of mechanisms corresponding to arbitrary queries under TPMDP settings. Although the comparison with LDP mechanisms~\cite{kairouz2015secure} and PDP mechanisms~\cite{jorgensen2015conservative} is important, the utility of such mechanisms heavily depends on the specific query functions, whence generic results cannot be obtained. We plan to compare the utility of our mechanism with those mechanisms for some common query functions, e.g., COUNT, SUM, and some machine learning tasks, as part of future research.
}

\comment{
\textbf{Generalization of TPMDP to the malicious setting}: Another future direction is to generalize TPMDP to settings where involved parties can be malicious, i.e., parties may provide bad inputs. It becomes challenging to devise a mechanism with high utility in such settings, while it is still possible to reduce the effect of such bad inputs on the utility for some specific applications. For example, in sensor fusion tasks~\cite{mitchell2007multi}, one may average out the effect of bad inputs if the sensors are sufficiently numerous and most of them behave honestly.
}

\hide{
\textbf{Adversarial model and communication cost.} The communication cost of Alg.~\ref{alg:DP_Gaussian} mainly depends on the underlying MPC protocol $\pi$. In this paper, we only assume that $\pi$ is secure (cf. Definition~\ref{def:c_MPC}). 
We plan to investigate the communication cost when applying Alg.~\ref{alg:DP_Gaussian} on concrete applications. Another future direction is to generalize TPMDP to settings where involved parties are malicious.
}

\hide{
\textbf{Algorithm for statistical and computational case.}
By Theorem \ref{thm:DP_multi_Gaussian_perf}, Eq.~\eqref{eq:DP_multi_Gaussian} is the necessary and sufficient condition for a multi-party Gaussian mechanism $\Pi$ to be perfectly $(\tau, n, \mathcal{E})$-TPMDP when the MPC protocol in $\Pi$ is perfectly $t$-private and $\tau\leq t$. Thus $\boldsymbol{\sigma}$ obtained from Alg. \ref{alg:DP_OPS_2} in this case is optimal. For the statistical case, Theorem \ref{thm:DP_multi_Gaussian_stat} shows that Eq.~\eqref{eq:DP_multi_Gaussian_stat} gives the tight bound on $\boldsymbol{\sigma}$. We observe that there exists a discrepancy between Eq.~\eqref{eq:DP_multi_Gaussian} and Eq.~\eqref{eq:DP_multi_Gaussian_stat}, which implies that $\boldsymbol{\sigma}$ obtained from Alg. \ref{alg:DP_OPS_2} is is suboptimal in this case. However, we can use exactly the same algorithm to derive a better solution in this case by adding a negligible term (e.g., $\exp{(-\left|\bar{x}\right|)}$) to $\delta_i$ for $i\in \{1,\hdots,n\}$. For the computational case, we only provide a sufficient condition, cf. Eq.~\eqref{eq:DP_multi_Gaussian_stat}. 
However, it holds that Eq.~\eqref{thm:DP_multi_Gaussian_perf} is an asymptotic tight bound for the statistical and computational case. For the statistical case, one can verify that the gap between Eqs.~\eqref{thm:DP_multi_Gaussian_perf} and \eqref{thm:DP_multi_Gaussian_stat} tends to zero as $\left|\bar{x}\right|$ increases. For the computational case, as $\left|\bar{x}\right|$ tends to infinity, RHS's of Eqs.~\eqref{eq:poly_ind} and \eqref{eq:s_ind} tend to be equal when entries of $X$ and $Y$ are i.i.d, which implies that the sufficient condition for the computational case boils down  that for the statistical case.
}
%For computationally $(\tau, n, \mathcal{E})$-TPMDP multi-party Gaussian mechanism, the sufficient condition presented in Theorem \ref{thm:DP_multi_Gaussian_comp} is the same as the one in Theorem \ref{thm:DP_multi_Gaussian_stat}, which implies we can also improve $\boldsymbol{\sigma}$ in Alg. \ref{alg:DP_OPS_2} with a negligible term. 
%However, it is a non-trivial task to derive the necessary condition corresponding to Theorem \ref{thm:DP_multi_Gaussian_comp}, we are not sure whether the gap tends to zero as $\left|\bar{x}\right|$ increases. We also leave this as an open problem.

%With slight abuse of notations, we also refer $h(E)$ to the sorted tuple of $h(E)$.

%For an arbitrary set $E\subset U$, define $F^{(E)} = (F_i(\cdot))_{i\in h(E)}$. Then for $i\in A$, $A\in \mathcal{A}_\tau$ the $i$-th partial $l_2$ sensitivity corresponding to $F^{(A)}$ is defined as
%$$
%    \Delta_{2,i} F^{(A)} = \mathop{\max}\limits_{\mathop{x,y\in{(\{0,1\}^*)^n}}\limits_{x\overset{i}{\simeq} y}} \left\|F^{(A)}(x)-F^{(A)}(y)\right\|_2.
%$$

%Multi-party Gaussian mechanism in this case demands that each party computes a Gaussian distribution $\mathcal{N}(0, \sigma_i^2 I_{|F^{(U)}|})$ and samples a random noise $X_i$ from $\mathcal{N}(0, \sigma_i^2 I_{|F^{(U)}|})$ where $I_{|F^{(U)}|}$ denotes the identity matrix with the same dimension as $F^{(U)}(\cdot)$. Then all parties execute an MPC protocol with inputs $\bar{x}$, $\bar{X}$ and an output $M'_j(\bar{x},\bar{X}) = F_{h(j)}(\bar{x})+\Sigma_{i=1}^n X_i^{h(j)}$ to $u_j$ for $j\in U$ where $X_i^{h(j)}$ stands for the noise added to $F_{h(j)}$ by $u_j$.

%We can similarly prove that a multi-party Gaussian mechanism in this generalized case would be $(\tau,n,\mathcal{E})$-TPMDP if we replace $\Delta_{2,i} F$ by $\Delta_{2,i} F^{(A)}$ and replace $*\mathcal{A}_\tau$ by $\mathcal{A}_\tau$ in Theorem \ref{thm:DP_multi_Gaussian}. Notice that in this general case we do not define the active set as we regard $\perp$ as a special function here.

%Further we can similarly prove that optimize a multi-party Gaussian mechanism in this generalized case with respect to any valid loss functions is equivalent to optimizing it with respect to the variance while the optimization formula is given by Eq.~\eqref{eq:Gauss_opt} by replacing $\Gamma_j$ by $(\epsilon_j,\delta_j,\Delta_{2,j} F^{(A)})$. Although this is still an LP, it is more complex than the one where the query function is in the less general form as $\sigma_{(\epsilon_j,\delta_j,\Delta_{2,j} F^{(A)})}$ can be different for different $A$. Thus the results in Section \ref{sec:res} cannot be trivially generalized to this case. We leave whether there exists an efficient algorithm or under which conditions would there exists an efficient algorithm for this general case as an open problem.

%In this case, a computationally (statistically, perfectly ) refined query function for each $A\in \mathcal{A}_\tau$ (or $\mathcal{A}$), denoted by $F_A$ is defined as a function satisfying that there exists a probabilistic polynomial-time $\mathcal{S}$ such that $\{\mathcal{S}(F_A(\bar{x}))\}_{\bar{x}\in (\{(0,1)\}^*)^n}$ is computationally (statistically, perfectly ) indistinguishable from $\{(f_i(\bar{x}))_{i\in A}\}_{\bar{x}\in (\{(0,1)\}^*)^n}$. Then we can similarly prove that the generalized multi-party Gaussian mechanism is computationally (statistically, perfectly) $(\tau,n,\mathcal{E})$-TPMDP if


==> performance_1.tex <==
In this section, we analyze the utility and efficiency of our algorithm for the multi-party Gaussian mechanism. 
Our results show that the utility of our mechanism lies strictly between a centralized mechanism and a TMDP mechanism under heterogeneous privacy budgets and is much better than a heuristic approach with $\tau = n-1$, especially when $\tau$ is relatively small compared with $n$. 
We also show that Alg. \ref{alg:DP_OPS_2} substantially outperforms the state-of-the-art generic LP solver with respect to running time and storage.

%\vspace{-0.1in}
\subsection{Utility Analysis}

To analyze the utility loss of our proposed algorithm for the multi-party Gaussian mechanism (cf. Alg. \ref{alg:DP_OPS_2}), denoted by $G$, we introduce the following {three baselines}:

%\begin{itemize}
    \textbullet \textbf{\emph{MAX}}: It is an upper (utility loss) baseline that takes $\boldsymbol{\sigma}$ as $(\sigma_{\Gamma_j})_{j\in U}$ if $\left| *U \right| \geq 2$ and takes $(\sigma_j)_{j\in \overline{*U}} = (\sigma_{\Gamma_j})_{j\in \overline{*U}}$, $\sigma_{1*} = 0$, otherwise. \emph{MAX} is just a special case in Alg. \ref{alg:DP_OPS_2} when $\tau = n-1$. 
This is a heuristic baseline as it holds that such $\boldsymbol{\sigma}$ is always feasible for $\tau\leq n-1$ and can be obtained in $\mathcal{O}(1)$ steps as proved in Theorem \ref{thm:case_general_rst}.
    
    \textbullet \textbf{\emph{MIN}}: It is a lower (utility loss) baseline. We degenerate our model to the centralized one considered in DP where exists a trusted third party who gathers the data from all parties, computes the query function with additive Gaussian noise, and then releases the results to the active parties. In this model, the optimal Gaussian noise is $\mathcal{N}(0, \sigma_{MIN}^2)$ where $\sigma_{MIN} = \max_{i\in U} {\sigma_{\Gamma_i}}$ if $\left| *U \right| \geq 2$ and $\sigma_{MIN} = \max_{i\in \overline{*U}} {\sigma_{\Gamma_i}}$ otherwise. 
    
    \textbullet \textbf{\emph{T-MAX}}: It is a variant of our multi-party Gaussian mechanism by setting the global privacy budget as the most stringent budget of all the parties, i.e., setting $\sigma_{\Gamma_i} = \max_{j\in U} \sigma_{\Gamma_j}$ for $i\in U$, {that degenerates to a TMDP mechanism}. \comment{Note that the variance selection of \emph{T-MAX} has the same computation complexity as $G$} as it needs $\mathcal{O}(n)$ steps to find the most stringent budget except for the case where $\left|*U\right|=1$ for $i\in *U$ (i.e., $u_i$ is the only active user) or $\tau = n-1$ (i.e., everyone except $u_i$ can collude), where our algorithm also only takes $\mathcal{O}(1)$ steps (cf. Theorem~\ref{thm:case_general_rst}).
%\end{itemize}

%The first is an upper baseline (denoted by \emph{MAX}) which takes $\boldsymbol{\sigma}$ as $(\sigma_{\Gamma_j})_{j\in U}$ if $\left| *U \right| \geq 2$ and takes $(\sigma_j)_{j\in \overline{*U}} = (\sigma_{\Gamma_j})_{j\in \overline{*U}}$, $\sigma_{1*} = 0$ otherwise. \emph{MAX} is just a special case in Alg. \ref{alg:DP_OPS_2} when $\tau = n-1$. 
%This is a heuristic baseline as it holds that this $\boldsymbol{\sigma}$ is always feasible for $\tau\leq n-1$ and can be obtained in $\mathcal{O}(1)$ steps as proved in Theorem \ref{thm:case_general_rst}.
%The second is a lower baseline (denoted by \emph{MIN}). We degenerate our model to the centralized one considered in DP where we assume that there exists a trusted third party who gathers the data from all parties, computes the query function with additive Gaussian noise and then releases the results to the active parties. In this model, the optimal Gaussian noise is $\mathcal{N}(0, \sigma_{MIN}^2)$ where $\sigma_{MIN} = \max_{i\in U} {\sigma_{\Gamma_i}}$ if $\left| *U \right| \geq 2$ and $\sigma_{MIN} = \max_{i\in \overline{*U}} {\sigma_{\Gamma_i}}$ otherwise. 

We use $v_G$, $v_{MAX}$, $v_{MIN}$, and $v_{T\text{-}MAX}$ to indicate the optimal utility loss for $G$, \emph{MAX}, \emph{MIN}, and \emph{T-MAX}, respectively;
$v_G$, $v_{MAX}$, and $v_{T\text{-}MAX}$ are the sums of noise variances in $G$, \emph{MAX} and \emph{T-MAX} and $v_{MIN} = \sigma_{MIN}^2$, which are summarized in Table~\ref{tab:utility}. 
\begin{table}[htbp]
\centering
{%\small
%\begin{center}
\begin{tabular}{ m{2.0cm} | >{\centering\arraybackslash} m{2.4cm} | >{\centering\arraybackslash} m{4.5cm} }
    \hline
    Mechanism & Case & Utility loss \\
    \hline
    \multirow{4}{*}{$G$} & Subcases~\ref{subcase_1}\&\ref{subcase_3} & $\Sigma_{i=1}^{\xi-1} \sigma_{\Gamma_i}^2 + (\frac{2n - \tau}{n - \tau} - \xi) \sigma_{\Gamma_{\xi}}^2$ \\
    \cline{2-3}
    \multirow{4}{*}{} & Subcase~\ref{subcase_2} & $\Sigma_{i=1}^{\xi-1} \sigma_{\Gamma_i}^2 + (\frac{2n - \tau - 1}{n - \tau} - \xi) \sigma_{\Gamma_{\xi}}^2$ \\
    \cline{2-3}
    \multirow{4}{*}{} & Subcase~\ref{subcase_4} & $\sigma_{\Gamma_1}^2$ \\
    \cline{2-3}
    \multirow{4}{*}{} & Subcase~\ref{subcase_5} & $\sigma_{\Gamma_1}^2 + \frac{\tau - 1}{n - \left| *U \right| - \tau +1} \sigma_{\Gamma_2}^2$ \\
    \hline
    \multirow{4}{*}{\emph{T-MAX}} & Subcases~\ref{subcase_1}\&\ref{subcase_3} & $\frac{n}{n - \tau} \sigma_{\Gamma_1}^2$ \\
    \cline{2-3}
    \multirow{4}{*}{} & Subcase~\ref{subcase_2} & $\frac{n - 1}{n - \tau} \sigma_{\Gamma_1}^2$ \\
    \cline{2-3}
    \multirow{4}{*}{} & Subcase~\ref{subcase_4} & $\sigma_{\Gamma_1}^2$ \\
    \cline{2-3}
    \multirow{4}{*}{} & Subcase~\ref{subcase_5} & $\frac{n - \left| *U \right|}{n - \left| *U \right| - \tau +1} \sigma_{\Gamma_1}^2$ \\
    \hline
    \multirow{2}{*}{\emph{MAX}} & Subcases~\ref{subcase_1}\&\ref{subcase_3}-\ref{subcase_5} & $\Sigma_{i=1}^{n} \sigma_{\Gamma_i}^2$ \\
    \cline{2-3}
    \multirow{2}{*}{} & Subcase~\ref{subcase_2} & $\Sigma_{i=1}^{n-1} \sigma_{\Gamma_i}^2$ \\
    \hline
    \multirow{1}{*}{\emph{MIN}} & Subcases~\ref{subcase_1}-\ref{subcase_5} & $\sigma_{\Gamma_1}^2$ \\
    %\multirow{2}{*}{\emph{MIN}} & Subcases~\ref{subcase_1}\&\ref{subcase_3}-\ref{subcase_5} & $\sigma_{\Gamma_1}^2$ \\
    %\cline{2-3}
    %\multirow{2}{*}{} & Subcase~\ref{subcase_2} & $\sigma_{\Gamma_1}^2$ \\
    \hline
\end{tabular}
\caption{Utility loss for $G$, \emph{MAX}, \emph{MIN}, \emph{T-MAX} (For Subcases~\ref{subcase_1}\&\ref{subcase_3}-\ref{subcase_5}, $\sigma_{i}$ denotes the $i$-largest elements in $\boldsymbol{\sigma}$ and $\xi$ is defined in Eq.~\eqref{eq:exact_param_xi}. In Subcase~\ref{subcase_2}, $\sigma_{\Gamma_i}$ is the $i$-th largest element in $\overline{*\boldsymbol{\sigma}}$ and $\xi$ is defined in Eq.~\eqref{eq:exact_param_xi} with $n\leftarrow n-1$ and $\tau \leftarrow \tau -1$).}\label{tab:utility}
%\end{center}
}
\end{table}


In the following, we show the relationship between $v_G$ and $v_{MAX}$/$v_{MIN}$/ $v_{T\text{-}MAX}$ as $n$ tends to infinity for {three} settings:
\begin{enumerate}
    \item \textbf{Setting 1}\label{setting_1}: given a fixed size of collusion $\tau\geq 1$;
    \item \textbf{Setting 2}\label{setting_2}: given a fixed rate of colluding parties $p\in (0,1)$, i.e., $\tau = \lfloor pn \rfloor$;
    \item \textbf{Setting 3}\label{setting_3}: given a fixed $C\in \mathbb{N}_+$ and $\tau = n - C$ for $n\geq C+1$.
\end{enumerate}

In some analysis, we need the following assumption which states that $\sigma_{\Gamma_i}^2,\, i\in U$ is uniformly upper and lower bounded by some non-zero constants.

\begin{assumption}\label{ass:sigma_bounded}
    There exist $c_l,c_u>0$ such that for all $i\in \{1,\hdots,n\}$, $c_l < \sigma_{\Gamma_i}^2 < c_u$ for $n\in \mathbb{N}_+$.
\end{assumption}

\hide{
As mentioned before, \emph{T-MAX} is a variant of $G$ where by taking $\sigma_{\Gamma_i} \equiv \sigma_{\Gamma_1}$ for all $i$. Then, it follows that $v_{G} \leq v_{T\text{-}MAX}$ but the gap between them can be zero when $\sigma_{\Gamma_i}$'s for $i\in U$ are equal. Thus, to exclude this non-interesting case, we assume that there exists a multiplicative gap between $\sigma_{\Gamma_1}^2$ and $\sigma_{\Gamma_2}$.
}

Without loss in generality, in the rest of this section, we assume that the parameters $U$ and $\boldsymbol{\sigma}$ satisfy that $\sigma_{\Gamma_i}$ is the $i$-th largest element in $\boldsymbol{\sigma}$ in Subcases~\ref{subcase_1}\&\ref{subcase_3}-\ref{subcase_5}, and is the $i$-th largest element in $\overline{*\boldsymbol{\sigma}}$ in Subcase~\ref{subcase_2}.
For the comparison with \emph{T-MAX}, a personalized privacy setting with heterogeneous privacy budgets~\cite{jorgensen2015conservative} is considered, which is parameterized by a multiplicative gap between $\sigma_{\Gamma_1}$ and $\sigma_{\Gamma_2}$ (as formalized in the following assumption).


\begin{assumption}\label{ass:multp_gap}
    There exists $r\in (0,1)$ such that $\sigma_{\Gamma_2}^2 / \sigma_{\Gamma_1}^2 \leq r$.
\end{assumption}

\begin{remark}
    It is worth noting that Assumption~\ref{ass:multp_gap} can be relaxed such that there exists $s\in \mathbb{N}_+$ and $r\in (0,1)$, and for $n\geq s$, $\sigma_{\Gamma_s}^2 / \sigma_{\Gamma_1}^2 \leq r$. Under such assumption, the relation between $v_{T\text{-}MAX}$ and $v_{G}$ is similar to that under Assumption~\ref{ass:multp_gap}. For simplicity, in the following, we just analyse $v_{T\text{-}MAX}/v_{G}$ under Assumption~\ref{ass:multp_gap}.
\end{remark}

The relations of $v_G$, $v_{T\text{-}MAX}$, $v_{MAX}$, and $v_{MIN}$ are presented in the following theorems. 
The proofs can be done by evaluating results in Table~\ref{tab:utility} under Settings~\ref{setting_1}-\ref{setting_3}. We omit the details for length considerations.

\begin{theorem}\label{thm:setting_1_bnd}
    For Setting~\ref{setting_1}, it holds that 
    $$
        %\left\{
        \begin{aligned}        
            \lim_{n\rightarrow +\infty} v_G / v_{MIN} = \lim_{n\rightarrow +\infty} v_{T\text{-}MAX} / v_{MIN} = \lim_{n\rightarrow +\infty} v_G / v_{T\text{-}MAX} = 1.
        \end{aligned}
        %\right.
    $$
    Under Assumption~\ref{ass:sigma_bounded}, it holds that for $n\geq 2\tau$,
    $$
        \frac{v_{MAX}}{v_{G}} \geq \frac{v_{MAX}}{v_{T\text{-}MAX}} \geq \left\{
        \begin{aligned}
            &\frac{c_l}{c_u} (n - \tau),\, &Subcases~\ref{subcase_1} - \ref{subcase_3}\&\ref{subcase_5} \\
            &\frac{c_l}{c_u} n,\, &Subcase~\ref{subcase_4}. \\
        \end{aligned}
        \right.
    $$
\end{theorem}

We proceed to give theorems corresponding to Settings~\ref{setting_2}\&\ref{setting_3}. Note that in both settings, Subcase~\ref{subcase_4} is not attainable where $\tau$ is fixed to $1$.

\begin{theorem}\label{thm:setting_2_bnd}
    For Setting~\ref{setting_2}, it holds that 
    $$
    \lim_{n\rightarrow +\infty} v_G / v_{MIN} \leq \lim_{n\rightarrow +\infty} v_{T\text{-}MAX} / v_{MIN} = \frac{1}{1-p}
    $$ for Subcases~\ref{subcase_1}-\ref{subcase_3}$\&$\ref{subcase_5}.
    Under Assumption~\ref{ass:multp_gap}, it holds that for Subcases~\ref{subcase_1}-\ref{subcase_3}$\&$\ref{subcase_5}, 
    $$
    \lim_{n\rightarrow +\infty} v_G / v_{MIN} \leq \frac{1 - (1 - r) p}{1 - p}
    $$ and 
    $$
    \lim_{n\rightarrow +\infty} v_G / v_{T\text{-}MAX} \leq 1 - (1 - r) p.
    $$ Under Assumption~\ref{ass:sigma_bounded}, it holds that for $n\geq \frac{1}{p(1-p)}$,
    $$
    {v_{MAX}}/{v_{G}} \geq {v_{MAX}}/{v_{T\text{-}MAX}} \geq \frac{c_l}{c_u} (1 - p)n,
    $$
    for Subcases~\ref{subcase_1}-\ref{subcase_3}$\&$\ref{subcase_5}.
\end{theorem}

\begin{theorem}\label{thm:setting_3_bnd}
    For Setting~\ref{setting_3}, it holds that for $n > 2C$, Subcase~\ref{subcase_5} is not attainable. For the other cases,
    $$
        \frac{v_{G}}{v_{MIN}} \leq \frac{v_{T\text{-}MAX}}{v_{MIN}} = \left\{
        \begin{aligned}
            &\frac{n}{C},\, &Subcases~\ref{subcase_1}\&\ref{subcase_3} \\
            &\frac{n-1}{C},\, &Subcase~\ref{subcase_2}. \\
        \end{aligned}
        \right.
    $$
    Under Assumption~\ref{ass:multp_gap}, it holds that
    $$
        \frac{v_{G}}{v_{MIN}} \leq \left\{
        \begin{aligned}
            &\frac{r}{C} n + 1 - r,\, &Subcases~\ref{subcase_1}\&\ref{subcase_3} \\
            &\frac{r}{C} (n-1) + 1 - r,\, &Subcase~\ref{subcase_2}, \\
        \end{aligned}
        \right.
    $$
    and
    $\lim_{n\rightarrow +\infty}{v_{G}}/{v_{T\text{-}MAX}} = r$.
    Under Assumption~\ref{ass:sigma_bounded}, it holds that for $n\geq 2 C$,
    $$
    {v_{MAX}}/{v_{G}} \geq {v_{MAX}}/{v_{T\text{-}MAX}} \geq \max\{1, \frac{c_l}{c_u} C\},
    $$
    for Subcases~\ref{subcase_1}-\ref{subcase_3}.
\end{theorem}

\comment{
\begin{remark}
    In this paper, we give bounds for utility ratios related to $r$, a ratio that reflects the heterogeneous privacy requirements parameterized by $\sigma_{\Gamma_i}^2$, which is uniquely determined by $(\epsilon_i, \delta_i)$.
    For bounds related to $(\epsilon_i, \delta_i)$, as posed in~\cite{balle2018improving}, $\sigma_{\Gamma_i}$ may vary substantially in terms of $\epsilon_i$ and $\delta_i$ in different regions of target $(\epsilon_i, \delta_i)$ (e.g., $\sigma_{\Gamma_i} = O(\min\{1/\delta_i, 1/\epsilon_i\}$) when $\epsilon_i\in (0, 1)$ whereas $\sigma_{\Gamma_i} = \Omega(1/\sqrt{\epsilon_i})$ for $\epsilon_i > 1$). Moreover, heterogeneous privacy budgets make the utility bounds related to $(\epsilon_i, \delta_i)$ more complicated.
    Thus, in this paper, we only consider the impact of privacy requirements on bounds parameterized by $\sigma_{\Gamma_i}$.
\end{remark}
}

\comment{We proceed to summarize results in Theorems~\ref{thm:setting_1_bnd}-\ref{thm:setting_3_bnd} in Table~\ref{tab:utility_bnd}. For clarification, we focus on the impact of $n$ and $r$ on the utility ratios in Settings~\ref{setting_1}-\ref{setting_3}, which correspond to the cases where the collusion size $\tau$ is constant, linear in $n$, and $n$ minus a constant.
}

\hide{
\begin{table}[h!]
\centering
{%\small
%\begin{center}
\begin{tabular}{ m{2.2cm} | >{\centering\arraybackslash} m{2.4cm} | >{\centering\arraybackslash} m{2.4cm} | >{\centering\arraybackslash} m{2.6cm} }
    \hline
    Ratio & Setting & Case & Asymptotic upper bound \\
    \hline
    \multirow{4}{*}{$\frac{v_G}{v_{MIN}}$} & \multirow{1}{*}{Setting~\ref{setting_1}} & Subcases~\ref{subcase_1}-\ref{subcase_5} & $1$ \\
    \cline{2-4}
    \multirow{4}{*}{} & \multirow{1}{*}{Setting~\ref{setting_2}} & Subcases~\ref{subcase_1}-\ref{subcase_3}\&\ref{subcase_5} & $\frac{1-(1-r)p}{1-p}$ \\
    \cline{2-4}
    \multirow{4}{*}{} & \multirow{2}{*}{Setting~\ref{setting_3}} & Subcases~\ref{subcase_1}\&\ref{subcase_3} & $\frac{r}{C}n+1-r$ \\
    \cline{3-4}
    \multirow{4}{*}{} & \multirow{2}{*}{} & Subcases~\ref{subcase_2} & $\frac{r}{C}(n-1)+1-r$ \\
    \cline{2-4}
    \hline
    \multirow{4}{*}{$\frac{v_{T\text{-}MAX}}{v_{MIN}}$} & \multirow{1}{*}{Setting~\ref{setting_1}} & Subcases~\ref{subcase_1}-\ref{subcase_5} & $1$ \\
    \cline{2-4}
    \multirow{4}{*}{} & \multirow{1}{*}{Setting~\ref{setting_2}} & Subcases~\ref{subcase_1}-\ref{subcase_3}\&\ref{subcase_5} & $\frac{1}{1-p}$ \\
    \cline{2-4}
    \multirow{4}{*}{} & \multirow{2}{*}{Setting~\ref{setting_3}} & Subcases~\ref{subcase_1}\&\ref{subcase_3} & $\frac{n}{C}$ \\
    \cline{3-4}
    \multirow{4}{*}{} & \multirow{2}{*}{} & Subcases~\ref{subcase_2} & $\frac{n-1}{C}$ \\
    \hline
    \multirow{3}{*}{$\frac{v_{G}}{v_{T\text{-}MAX}}$} & \multirow{1}{*}{Setting~\ref{setting_1}} & Subcases~\ref{subcase_1}-\ref{subcase_5} & $1$ \\
    \cline{2-4}
    \multirow{3}{*}{} & \multirow{1}{*}{Setting~\ref{setting_2}} & Subcases~\ref{subcase_1}-\ref{subcase_3}\&\ref{subcase_5} & $1 - (1-r)p$ \\
    \cline{2-4}
    \multirow{3}{*}{} & \multirow{1}{*}{Setting~\ref{setting_3}} & Subcases~\ref{subcase_1}-\ref{subcase_3} & $r$ \\
    \hline
    \multirow{3}{*}{$\frac{v_{G}}{v_{MAX}} (\frac{v_{T\text{-}MAX}}{v_{MAX}})$} & \multirow{2}{*}{Setting~\ref{setting_1}} & Subcases~\ref{subcase_1}-\ref{subcase_3}\&\ref{subcase_5} & $\frac{c_u}{c_l(n-\tau)}$ \\
    \cline{3-4}
    \multirow{4}{*}{} & \multirow{2}{*}{} & Subcases~\ref{subcase_4} & $\frac{c_u}{c_l n}$ \\
    \cline{2-4}
    \multirow{4}{*}{} & \multirow{1}{*}{Setting~\ref{setting_2}} & Subcases~\ref{subcase_1}-\ref{subcase_3}\&\ref{subcase_5} & $\frac{c_u}{c_l (1-p) n}$ \\
    \cline{2-4}
    \multirow{4}{*}{} & \multirow{1}{*}{Setting~\ref{setting_3}} & Subcases~\ref{subcase_1}-\ref{subcase_3} & $\min\{1, \frac{c_u}{c_l C}\}$ \\
    \hline
\end{tabular}
\caption{Asymptotic upper bounds for ratios related to $v_G$, $v_{T\text{-}MAX}$, $v_{MAX}$, and $v_{MIN}$ under Assumption~\ref{ass:sigma_bounded}\&\ref{ass:multp_gap}.}
\label{tab:utility_bnd}
%\end{center}
}
\end{table}
}


\begin{table}[h!]
\centering
{%\small
%\begin{center}
\begin{tabular}{ m{2.2cm} | >{\centering\arraybackslash} m{2.4cm} | >{\centering\arraybackslash} m{4.3cm} }
    \hline
    Ratio & Setting & Asymptotic upper bound \\
    \hline
    \multirow{3}{*}{$\frac{v_G}{v_{MIN}}$} & Setting~\ref{setting_1} & $1$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_2} & $1 + \mathcal{O}(r)$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_3} & $\mathcal{O} (rn)$ \\
    \hline
    \multirow{3}{*}{$\frac{v_{T\text{-}MAX}}{v_{MIN}}$} & Setting~\ref{setting_1} & $1$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_2} & $\mathcal{O}(1)$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_3} & $\mathcal{O}(n)$ \\
    \hline
    \multirow{3}{*}{$\frac{v_{G}}{v_{T\text{-}MAX}}$} & Setting~\ref{setting_1} & $1$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_2} & $1 - \mathcal{O}(1-r)$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_3} & $r$ \\
    \hline
    \multirow{2}{*}{$\frac{v_{G}}{v_{MAX}} (\frac{v_{T\text{-}MAX}}{v_{MAX}})$} & Settings~\ref{setting_1}\&\ref{setting_2} & $\mathcal{O}(\frac{1}{n})$ \\
    \cline{2-3}
    \multirow{3}{*}{} & Setting~\ref{setting_3} & $\mathcal{O}(1)$ \\
    \hline
\end{tabular}
\caption{\comment{Asymptotic upper bounds for ratios related to $v_G$, $v_{T\text{-}MAX}$, $v_{MAX}$, and $v_{MIN}$ under Assumption~\ref{ass:sigma_bounded}\&\ref{ass:multp_gap} ($r$ is the multiplicative gap between $\sigma_{\Gamma_1}$ and $\sigma_{\Gamma_2}$, cf. Assumption~\ref{ass:multp_gap}).}}
\label{tab:utility_bnd}
%\end{center}
}
\end{table}




\begin{remark}
    The results stated in Theorem~\ref{thm:setting_1_bnd}-\ref{thm:setting_3_bnd} are summarized in Table~\ref{tab:utility_bnd}. From the table, we can conclude that \textbf{the utility of $G$ lies strictly between \emph{MAX} (\emph{T-MAX}) and \emph{MIN} in all the three settings}. Specially, \textbf{when $\tau$ is relatively small (i.e., Settings~\ref{setting_1}\&\ref{setting_2}), $\boldsymbol{v_G/v_{MIN}}$ is $\boldsymbol{\mathcal{O}(1)}$ while $\boldsymbol{v_{MAX}/v_{G}}$ is $\boldsymbol{\mathcal{O}(n)}$ (w.r.t. $\boldsymbol{n}$)}. When taking the impact of $\tau$ and $r$ into considerations, it holds that $v_G$ becomes closer to $v_{MIN}$ while farther away from $v_{MAX}$ as either $\tau$ or $r$ becomes smaller.
    When compared with \emph{T-MAX}, $G$ takes advantage of personalized budgets (i.e., $r$) more when the collusion size is relatively large (i.e., Settings~\ref{setting_2}\&\ref{setting_3}). Concretely, \textbf{in both Settings~\ref{setting_2}\&\ref{setting_3} $\boldsymbol{v_G/v_{T\text{-}MAX}}$ decreases linearly in $\boldsymbol{r}$ as $\boldsymbol{r}$ tends to zero}.
    \hide{
    From the table, we can conclude that when the size of collusion $\tau$ is constant or a constant ratio of $n$ \textbf{(i.e., Setting~\ref{setting_1}\&\ref{setting_2}), $\boldsymbol{v_G/v_{MIN}}$, $\boldsymbol{v_{T\text{-}MAX}/v_{MIN}}$, and $\boldsymbol{v_G/v_{T\text{-}MAX}}$ are $\boldsymbol{\mathcal{O}(1)}$ (w.r.t. $n$).} 
    When taking $p$ and $r$ into consideration, $v_G/v_{MIN}$ and $v_{T\text{-}MAX}/v_{MIN}$ increase while $v_{G} / v_{T\text{-}MAX}$ decreases with respect to $p$, and both $v_G/v_{MIN}$ and $v_{G}/v_{T\text{-}MAX}$ increases in $r$ in Setting~\ref{setting_2}.
    Also, \textbf{in both settings, $\boldsymbol{v_{MAX}/v_{G}}$ and $\boldsymbol{v_{MAX}/v_{T\text{-}MAX}}$ are $\boldsymbol{\mathcal{O}{(n)}}$.}
    Finally, if $n-\tau$ is constant (i.e., Setting~\ref{setting_3}), $v_{MAX}/v_{G}$ and $v_{MAX}/v_{T\text{-}MAX}$ turn to $\mathcal{O}{(1)}$ while  $v_G/v_{MIN}$ and $v_{T\text{-}MAX}/v_{MIN}$ become $\mathcal{O}(n)$ with respect to $n$ in this case.
    For the impact of $C$ and $r$, we can find that $v_G/v_{MIN}$ and $v_{T\text{-}MAX}/v_{MIN}$ decrease in $C$, and both $v_G / v_{MIN}$ and $v_{G} / v_{T\text{-}MAX}$ increases in $r$.
    To conclude, we find that the utility of $G$ is relatively close to \emph{MIN} while superior to \emph{MAX} if the collusion size is relatively small. The result reverses if the collusion size is very close to $n$.
    \textbf{When compared with \emph{T-MAX}, $\textbf{G}$ takes advantage of personalized budgets (i.e., $\textbf{r}$) more when the collusion size is relatively large.}
    }
\end{remark}

\hide{
\begin{theorem}\label{thm:v_G_lo}
    For Settings~\ref{setting_1}\&\ref{setting_2}, $v_G / v_{MIN} = \mathcal{O}(1)$.
\end{theorem}


\begin{theorem}\label{thm:v_up_O}
    For Settings \ref{setting_1}\&\ref{setting_2}, if there exists a constant $c>0$ such that $\min_{i\in U} \sigma_{\Gamma_i} / \max_{i\in U} \sigma_{\Gamma_i} \geq c$, then $v_{MAX} / v_G = \mathcal{O}(n)$.
\end{theorem}

{These two theorems state that, in both settings, the utility of our proposed mechanism $G$ is ``close'' to that of the centralized mechanism \emph{MIN}, while it is much better than that of the heuristic approach \emph{MAX}.}
}

\hide{
An equivalent condition to that in Theorem \ref{thm:v_up_O} (i.e., $\min_{i\in U} \sigma_{\Gamma_i} / \max_{i\in U} \sigma_{\Gamma_i} \geq c$) is that there exist non-zero uniform upper and lower bounds for $\sigma_{\Gamma_i}$ for $i\in U$. In our experiments, we always assume that this condition holds.
}

\hide{
\begin{figure*}[h!]
\centering
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth]{fig/cnt_density_n1000_tau25_case1_(density).png}
\caption{Impact of $\rho$}\label{fig:cnt_a}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth]{fig/cnt_density_n1000_tau25_case1_(epsilon_c).png}
\caption{Impact of $\epsilon_C$ (with $\epsilon_M = 0.5$)}\label{fig:cnt_b}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth]{fig/cnt_density_n1000_tau25_case1_(f_c).png}
\caption{Impact of $f_C$}\label{fig:cnt_c}
\end{subfigure}

\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth]{fig/cnt_density_(n)_tau_25_case1_delta10ndiv.png}
\caption{Impact of $n$ (Setting \ref{setting_1})}\label{fig:cnt_d}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth]{fig/cnt_density_(n)_tau_np_case1_delta10ndiv.png}
\caption{Impact of $n$ (Setting \ref{setting_2})}\label{fig:cnt_e}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth]{fig/cnt_density_n1000_(tau)_case1.png}
\caption{Impact of $\tau$}\label{fig:cnt_f}
\end{subfigure}
\caption{Utility loss for count 
{($G$ is our proposed mechanism; \emph{MIN} and \emph{MAX} are centralized and heuristic baselines, respectively; $S_{avg}$ and $S_{MAX}$ are two variants of Sample mechanisms; $L$ stands for randomized response. From Fig. \ref{fig:cnt_a} to Fig. \ref{fig:cnt_e}, the curves for \emph{MIN} are overlapped with that for $G$.)}}\label{fig:cnt}
\vspace{-0.15in}
\end{figure*}

\vspace{-0.15in}
\subsection{Experimental Evaluation of Utility Loss}
\vspace{-0.1in}

\textbf{Experimental setup}: We demonstrate the utility loss of our proposed mechanism for two common query functions count and linear regression. Count/sum is a fundamental operation in complex data analytic tasks. Linear regression is widely adopted in various data analytic systems. The utility loss of the mechanism is measured using rooted mean squared error (RMSE). Besides \emph{MIN} and \emph{MAX}, we also compare our mechanism with the following two personalized differential privacy mechanisms:
\hide{
we also compare our mechanism with
\comment{a state-of-the-art centralized PDP mechanism~\cite{jorgensen2015conservative}, a randomized response mechanism~\cite{kairouz2015secure} (for count) and the non-private mechanism (for linear regression).}:}
%\begin{itemize}

\textbullet \textbf{\emph{Sample}~\cite{jorgensen2015conservative} (including two variants $S_{max}$ and ${S_{avg}}$)}: It is a state-of-the-art centralized PDP mechanism. 
{
%which performs particularly well for several applications. 
The basic idea is seeking to eliminate data requiring stringent privacy guarantees with high probability. Hence, the perturbation required by the mechanism can be reduced.} For the privacy budgets $\mathcal{E} = ((\epsilon_i,\delta))_{i\in U}$, it introduces two independent sources of randomness: 1) given a threshold $\epsilon^{(t)} > 0$, it independently samples $x_j$ with probability $\pi_j$ for $j\in U$, where
$$
\pi_j = \left\{
    \begin{aligned}
        \frac{\exp{(\epsilon_j)} - 1}{\exp{(\epsilon^{(t)})} - 1}, \quad if\, \epsilon_j < \epsilon^{(t)} \\
        1, \quad otherwise.
    \end{aligned}
    \right.
$$
2) it invokes a traditional DP mechanism on the sampled data with privacy budget $(\epsilon^{(t)}, \delta)$.
%Although the original Sample mechanism is defined in the setting where the privacy budgets are parameterized by $\epsilon_i$, $i\in U$, it can be generalized to the setting where the privacy budgets are parameterized by $(\epsilon_i, \delta)$, $i\in U$ by invoking a $(\epsilon^{(t)}, \delta)$-DP mechanism in the second step. 
Similar to~\cite{jorgensen2015conservative}, we take $\epsilon^{(t)} = \max_{i\in U} \epsilon_i$ and $\epsilon^{(t)} = \frac{1}{n} \Sigma_{i\in U} \epsilon_i$ respectively for two variants $S_{max}$ and ${S_{avg}}$. 

\textbullet  \textbf{Randomized response LDP~\cite{kairouz2015secure} (denoted by $L$)}: We also introduce the personalized multi-party non-interactive LDP mechanism as a baseline (\comment{Randomized response for count and input perturbation for Linear regression}).

\textbullet \textbf{Non-private linear regression algorithm (denoted by \emph{non-private})}: For the case of Linear Regression, we additionally compare our mechanism with the the non-private linear regression algorithm.
%\end{itemize}


\textbf{Datasets}: We evaluate mechanisms for count on synthetic data. We sample a dataset with $n$ records (default $n=1000$), each with a single binary attribute. 
The fraction of `$1$''s in the dataset is controlled by a density parameter $\rho$ ($\rho = 0.15$ by default). 
For linear regression, we use a real-world \comment{revenue} dataset containing $5$ features \comment{(number of children, sex, age, educational level, and annual income (for prediction))} and $2.5\times 10^6$ records~\cite{ipums} (by default, we take $n = 2\times 10^5$ data for training) and each attribute of the dataset is normalized in the range $[-1,1]$. In each experiment, the data are randomly distributed to all parties.








\textbf{Privacy budgets}: Similar to~\cite{jorgensen2015conservative}, \comment{based on a social investigation on people's privacy concerns~\cite{AcquistiG05}}, we randomly divide the parties into three groups: 1) conservative, representing parties with high privacy consideration; 2) moderate, representing parties with medium consideration; 3) liberal, with low consideration. The fractions of conservative and moderate parties are denoted by $f_C$ and $f_M$ respectively. Consequently, the fraction of liberal parties is $1-f_C-f_M$, denoted by $f_L$. The default values for $f_C$ and $f_M$ are $0.54$ and $0.37$~\cite{jorgensen2015conservative}. As for the set of privacy budgets $\mathcal{E}$, \comment{we choose $\delta_i = \frac{1}{10n}$ for $i\in U$ as it is advisable to choose $\delta$ a small multiple of $\frac{1}{n}$~\cite{abadi2016deep}}. Values for $\epsilon$'s for parties in conservative and moderate groups are chosen uniformly at random from $[\epsilon_C, \epsilon_M]$ and $[\epsilon_M, \epsilon_L]$, respectively, while $\epsilon$'s for liberal parties are fixed to $\epsilon_L$. The default values for $\epsilon_C$, $\epsilon_M$, and $\epsilon_L$ are $0.01$, $0.2$, and $1.0$.



\begin{figure*}[h]
\centering

\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth,height=1.3in]{fig/linear_reg_n200000_tau25_case1_(epsilon_c)_delta10ndiv.png}
\caption{Impact of $\epsilon_C$ (with $\epsilon_M = 0.5$)}\label{fig:linReg_a}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth,height=1.3in]{fig/linear_reg_n200000_tau25_case1_(f_c)_delta10ndiv.png}
\caption{Impact of $f_C$}\label{fig:linReg_b}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth,height=1.3in]{fig/linear_reg_(n)_tau_25_case1_delta10ndiv.png}
\caption{Impact of $n$ (Setting \ref{setting_1})}\label{fig:linReg_c}
\end{subfigure}

\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth,height=1.3in]{fig/linear_reg_(n)_tau_np_case1_delta10ndiv.png}
\caption{Impact of $n$ (Setting \ref{setting_2})}\label{fig:linReg_d}
\end{subfigure}
%
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\linewidth,height=1.3in]{fig/linear_reg_n200000_(tau)_case1_delta10ndiv.png}
\caption{Impact of $\tau$}\label{fig:linReg_e}
\end{subfigure}
\caption{Utility loss of different mechanisms for linear regression (From Fig. \ref{fig:linReg_a} to Fig. \ref{fig:linReg_d}, the curves for \emph{MIN} is partially or totally overlapped by the ones for $G$. In all figures, the curves for $S_{min}$ is overlapped by that for $S_{max}$).}\label{fig:linReg}
\vspace{-0.15in}
\end{figure*}


\textbf{Results for count}: Fig. \ref{fig:cnt} presents the utility of different mechanisms for the count query. 
$*U$ is chosen randomly from the subsets of $U$. 
We perform each mechanism for each configuration over 1000 times and present average results. 
Overall, the utility of \emph{MAX} is significantly worse than others.   
When $\tau = 25$ (by default) the utility loss curves for $G$ are overlapped with curves of \emph{MIN} in all cases in Figs. \ref{fig:cnt_a} to \ref{fig:cnt_e}, 
which shows that our mechanism $G$ achieves the same utility as \emph{MIN} and outperforms other mechanisms in most cases.

\emph{1) Impact of data density:} Fig. \ref{fig:cnt_a} shows that the utility loss of $G$, \emph{MIN}, and \emph{MAX} stay unchanged with regards to varying data density $\rho$, 
while the utility loss of $S_{max}$ and $S_{avg}$ increases linearly in $\rho$. 
This can be explained in light of the fact that for smaller values of $\rho$ most of the data discarded by the Sample mechanism are $0$'s, resulting in little accuracy loss.
For larger $\rho$'s, however, the Sample mechanism ignores too many $1$'s and makes a larger count error. 
Utility loss for the randomized response mechanism $L$ is the smallest when $\rho$ is about $0.5$, however it becomes large when $\rho$ is approaching $0$ or $1$. 
The reason is that when the testing data obey a Bernoulli distribution $B(n, \rho)$, the operation of randomized response is equivalent to $\mathop{xor}$.
Based on the property of $\mathop{xor}$, it holds that when $\rho = 0.5$ the perturbed inputs follow the same distribution as the raw testing data, i.e., $B(n, \rho)$,
thus the noise does not incur significant count error. 
When $\rho$ equals to $0$ or $1$, the mean squared error equals to the the sum of the variances of the noise, thus the RMSE values for the randomized response in these two cases are comparatively large. 
%Next, in  and Fig. \ref{fig:cnt_c}, we present the resulting RMSE's when varying the privacy parameters $\epsilon_C$ and $f_C$ respectively. Note that 

\emph{2) Impact of privacy budget:} In Fig. \ref{fig:cnt_b}, the privacy budget $\epsilon_C$ varies from $0$ to $0.5$ to ensure that $\epsilon_C \leq \epsilon_M$ as required in the generation of privacy budgets. 
%From the plot in Fig. \ref{fig:cnt_b}, 
The utility loss of $S_{max}$ and $S_{avg}$ is not sensitive to $\epsilon_C$, 
since the additive noises of the Sample mechanisms are determined by $\epsilon^{(t)}$, which is much larger than $\epsilon_C$.
For $L$, its utility loss decreases slowly as $\epsilon_C$ increases due to the fact that it maps $\{0,1\}$ back to $\{0,1\}$ using a specified probability measure instead of adding noise directly.
Differently, the utility loss of \emph{MAX}, \emph{MIN} and $G$ is large when $\epsilon_C$ is very close to $0$ and declines sharply as $\epsilon_C$  gets larger. 
The reason is that the noises of the Gaussian mechanisms are directly determined by the privacy budgets, which diminish fast as $\epsilon_C$ increases. 
When $\epsilon_C>0.05$, $G$ and \emph{MIN} perform best and achieve a very small and stable utility loss over variable values of $\epsilon_C$.
%which makes the resulting error not that sensitive to the privacy budgets comparing to Gaussian mechanisms. 
%Also from the plot, $G$ is the best mechanism with respect to RMSE when $\epsilon_C \geq 0.1$. 


\emph{3) Impact of fraction of conservative users:} Fig. \ref{fig:cnt_c} depicts that except for \emph{MAX}, other mechanisms are not sensitive to 
%the fraction of conservative users 
$f_C$. 
$G$ ranks third among the mechanisms, which is slightly worse than $S_{max}$ and $S_{avg}$, and the gaps between $G$ and these two Sample mechanisms decrease as $f_C$ increases.
%Although $S_{avg}$ is always the best mechanism, the gap between the RMSE of $G$ and that of $S_{avg}$ is below $150$ for most $f_C$'s.

\emph{4) Impact of number of parties:} Figs. \ref{fig:cnt_d} and \ref{fig:cnt_e} illustrate the impact of the number of parties $n$ in Setting~\ref{setting_1} and Setting~\ref{setting_2}, respectively. 
In both settings,  $G$ and \emph{MIN} attain the lowest utility loss and remain unchanged as $n$ increases.
Other mechanisms suffer from an increasing utility loss when $n$ gets larger. 
In particular, the increase of utility loss for $S_{max}$, $S_{avg}$ and $L$ is linear in $n$. 
Because, for $S_{max}$ and $S_{avg}$, the data discarded by the Sample mechanisms linearly increase with $n$; for $L$, the number of inputs mapping to the opposite ones linearly increase with $n$.
%the ranking of the six mechanisms' RMSE's from the largest to the smallest is \emph{MAX}, $L$, $G$, \emph{MIN}, $S_{max}$ and $S_{avg}$ for small $n$ and the ranking turns to be \emph{MAX}, $L$, $S_{max}$, $S_{avg}$, $G$ and \emph{MIN} when $n>3000$. Also, the utilities of $G$ and \emph{MIN} are close and won't change much as $n$ increases while RMSE of \emph{MAX} increases fast as $n$ tends to infinity. 
These results are consistent with our theoretical analysis in Theorems \ref{thm:v_G_lo} and \ref{thm:v_up_O}. 

%For the other three mechanisms, we can find that RMSE's of those mechanisms increase linearly as $n$ increases. For $S_{max}$ and $S_{avg}$, this is because the data discarded by the Sample mechanism linearly increase as $n$ increases and for $L$, this is because the number of inputs mapping to the opposite ones linearly increase.
\emph{5) Impact of number of corrupted parties:} Fig. \ref{fig:cnt_f} examines the impact of $\tau$ and shows that except for $G$, other mechanisms are not sensitive to changes of $\tau$, since $G$ is the only mechanism considering different thresholds. 
The utility loss of $G$ is close to that of $\emph{MIN}$ for $\tau<300$ and remains better than that of $L$ when $\tau<600$. 
When $\tau$ is greater than $800$, the utility of $G$ deteriorates sharply, as in this case, the threshold in $G$ is close to $n-1$ (which is the threshold for \emph{MAX}).


\hide{
\begin{figure*}[ht]
\centering
\begin{subfigure}[t]{0.3\textwidth}
\centering
\includegraphics[width=0.85\linewidth,height=1.3in]{fig/space_comp_(n).png}
\caption{Comparison of space requirement}\label{fig:eff_a}
\end{subfigure}
%
\begin{subfigure}[t]{0.3\textwidth}
\centering
\includegraphics[width=0.85\linewidth,height=1.3in]{fig/gurobi_efficiency_(n).png}
\caption{Comparison of execution time}\label{fig:eff_b}
\end{subfigure}
%
\begin{subfigure}[t]{0.3\textwidth}
\centering
\includegraphics[width=0.85\linewidth,height=1.3in]{fig/efficiency_(n).png}
\caption{Execution time of Alg. \ref{alg:DP_OPS_2}}\label{fig:eff_c}
\end{subfigure}
\caption{Efficiency evaluation (For Figs. \ref{fig:eff_a} \& \ref{fig:eff_b}, the first four curves are for Gurobi and the last one is for Alg. \ref{alg:DP_OPS_2} in setting \ref{setting_2} with $p = 0.5$; the run-time of Alg. \ref{alg:DP_OPS_2} in both settings is linear, and visually indiscernible, cf. Fig. \ref{fig:eff_c}).}\label{fig:eff}
\vspace{-0.15in}
\end{figure*}
}


\textbf{Results for linear regression}:
%thus for these query functions and DP mechanisms satisfying that Eq.~\eqref{eq:DP} holds for all $x,y$ where $\left \| f(x) - f(y) \right \| \leq \Delta f$ (e.g. Laplace, Gaussian and Exponential mechanisms~\cite{dwork2014algorithmic}), Sample mechanism can be similarly proved to satisfy $\mathcal{E}$-PDP if replacing $\overset{j}{\approx}$ by $\overset{j}{\simeq}$ for $j\in U$.
%
%
%Next, we compare the utility of our algorithm with these two baselines on concrete query functions.
%
For linear regression, we apply the Functional mechanism in \cite{zhang2012functional}, whence the resulting weight of the linear regression is
\begin{equation}\label{eq:ppLR}
    w = (D^TD+X^{(1)}+4\sigma I)^{-1}(D^TY+X^{(2)}),
\end{equation}
where $\sigma$ is the standard deviation of the Gaussian mechanism with $\Delta_2 f = \sqrt{2d^2 + 15d}$, $D$ and $Y$ respectively correspond to data and labels, $X^{(1)}$ is a symmetric random matrix, and $X^{(2)}$ is a random vector.
Elements of $X^{(2)}$ and the upper triangular part of $X^{(1)}$ are i.i.d and the elements of $X^{(1)}$ obey $\mathcal{N}(0,\sigma^2)$ while the elements of $X^{(2)}$ obey $\mathcal{N}(0,\sigma^2/4)$~\cite{zhang2012functional}. 
\hide{
\comment{The goal of the Functional mechanism is to protect the objective function, which means the resulting mechanism is still TPMDP if it outputs $D^TD+X^{(1)}+4\sigma I$ and $D^TY+X^{(2)}$ instead of $w$, which makes the design of the underlying MPC protocol easier. Note that in Eq.~\eqref{eq:ppLR}, both $D^TD$ and $D^TY$ can be computed in a distributed manner without interaction (i.e., $D^TD = \Sigma_{i=1}^n D_i^TD_i$ and $D^TY = \Sigma_{i=1}^n D_i^TY_i$). Consequently, as in \emph{MAX}, both $X^{(1)}$ and $X^{(2)}$ can also be added in a distributed manner, \emph{MAX} can be done in an LDP manner, that is why we do not compare our mechanism with other LDP mechanisms.}
}
For each experiment, we perform 100 runs of five-fold cross-validation.

Similar to the experiments for count, we analyze the impact of $\epsilon_C$, $f_C$, $n$, and $\tau$ on utility loss for different mechanisms and present results in Fig. \ref{fig:linReg}. 
In five sub-figures, the ranking of five mechanisms remains the same, which is \emph{non-private},  ($S_{avg}$ and $S_{max}$), ($G$ and \emph{MIN}), \emph{MAX}. 
In all cases, \emph{MAX} still has the largest utility loss;
$G$ has very similar performance as \emph{MIN};
$S_{max}$ and $S_{avg}$ have the minimum utility loss, which is close to the one of \emph{non-private}. 
This is partially because performing the linear regression algorithm on a randomly sampled dataset usually generates a similar model as that on the original dataset if the sample ratio is sufficiently high.
%which implies the sample operation in the Sample mechanism won't introduce much bias error.
Besides, the additive noise variance in the Sample mechanism is much smaller than that in the other three mechanisms.
%which together makes the Sample mechanism perform extreme well for linear regression.
%On the other hand, from Fig. \ref{fig:linReg_a} to Fig. \ref{fig:linReg_d}, RMSE's of \emph{MAX} are the largest
%On the other hand, in all five figures, \emph{MAX} is the worst mechanism with respect to RMSE among the five mechanisms.
%The observation regarding Fig. \ref{fig:linReg_a} and Fig. \ref{fig:linReg_b} illustrates that for linear regression, \emph{MAX} performs much worse than the other four mechanisms across all $\epsilon_C$'s and $f_C$'s as the additive noise is much larger than those of the other ones.
%For \emph{MAX}, \emph{MIN} and $G$, the corresponding RMSE's become smaller as $\epsilon_C$ increases.

\emph{1) Impact of privacy budget:} In Fig. \ref{fig:linReg_a}, except for \emph{MAX}, all other mechanisms have similarly low utility loss, and the utility loss of $G$ decreases as $\epsilon_C$ increases.

%and for $S_{max}$ and $S_{avg}$, their RMSE's are not sensitive to $\epsilon_C$ as the additive noise of the Sample mechanism is not sensitive to $\epsilon_C$. 
\emph{2) Impact of fraction of conservative users:} Fig. \ref{fig:linReg_b} shows that the utility loss of all five mechanisms is not sensitive to changes of $f_C$. 
For \emph{MIN}, $G$, $S_{max}$, and $S_{avg}$, this is attributed to that additive noises of these mechanisms do not increase fast with $f_C$.
For \emph{MAX}, this phenomenon is due to the fact that when the noise variance is very large, $w$ tends to a random vector independent of the training data 
%and RMSE gets close to $1$ 
(cf. Eq.~\eqref{eq:ppLR}).

\emph{3) Impact of number of parties:} Figs. \ref{fig:linReg_c} \& \ref{fig:linReg_d} present the impact of $n$ in Settings \ref{setting_1} \& \ref{setting_2}, respectively. 
\comment{In both settings, the utility loss for all mechanisms except for \emph{MAX} roughly decreases as $n$ increases, since the accuracy increase due to more training data exceeds the error caused by additive noise, while the fluctuation of loss for $G$ / \emph{MIN} around $n = 1.6\times 10^5$ is because the accuracy increase due to more training data does not dominate the noise if $n$ is not sufficiently large.}
%while for \emph{MAX}, the error reduction caused by the increase in the training set won't exceed the increase in additive noise.

\emph{4) Impact of number of corrupted parties:} Fig. \ref{fig:linReg_e} shows the impact of $\tau$. 
%Similar as the result for count, only $G$ is influenced by the change of $\tau$. 
When $\tau \leq 2500$, the utility loss of $G$ is very close to that of \emph{MIN}.
As $\tau$ getting larger, the utility of  $G$ increases and sharply reaches \emph{MAX} when $\tau$ tends to $n-1$.
}

%\vspace{-0.15in}
\subsection{Scalability Analysis}\label{subsec:scala}

As the original formulation for the LP (cf. Eq.~\eqref{eq:Gauss_opt}) contains many redundant constraints, we replace the constraints by the equivalent but more compact ones suggested by Corollary~\ref{cor:DP_min2} in Appendix~\ref{app:res} {where the number of constraints is $\mathcal{O} (n\binom{n-1}{\tau})$ and the LHS of each constraint is a summation of $n-\tau$ terms}. {We also evaluate the space complexity of describing the LP as input of a Mathematical Programming System (MPS)~\cite{cplex2009v12}.}
\hide{
Subsequently, we format the LP as the input of Mathematical Programming System (MPS) and invoke a generic LP solver to obtain the solution. 
}
Table \ref{tab:complexity} summarizes the space and time complexity for the generic LP solver and Alg. \ref{alg:DP_OPS_2} in both Settings \ref{setting_1} \& \ref{setting_2}.
%where the space complexity is evaluated using the size of the program as well as the MPS file and the time complexity is suggested in~\cite{lee2019solving}. 
The results for the generic LP solver are based on Eq.~\eqref{eq:DP_min2} and the time complexity in~\cite{lee2019solving} (i.e., $\widetilde{\mathcal{O}}((nnz(C)+rank(C)^2)\sqrt{rank(C)}\log{(1/\epsilon)})$), after a plain application of Stirling's formula.
Our algorithm achieves significant lower space and time complexity in both settings, with the gain being unbounded in the number of users. 


\begin{table}[htbp]
\centering
{%\small
%\begin{center}
\begin{tabular}{ m{3.4cm} | >{\centering\arraybackslash} m{3.0cm} | >{\centering\arraybackslash} m{4.5cm} }
    \hline
     & Space complexity & Time complexity \\
    \hline
    %\hline
    Generic LP solver for Setting \ref{setting_1} & $\mathcal{O}(n^{\tau+2})$ & $\widetilde{\mathcal{O}}(n^{\tau+2.5}) \log{(1/\epsilon)}$ \\
    \hline
    Generic LP solver for Setting \ref{setting_2} & $\mathcal{O}(n^{1.5} 2^{H(p)n})$ & $\widetilde{\mathcal{O}}(n^{2} 2^{nH(p)}) \log{(1/\epsilon)}$ \\
    \hline
    Generic LP solver for Setting \ref{setting_3} & $\mathcal{O}(n^C)$ & $\widetilde{\mathcal{O}}(n^{\max\{C+0.5,2.5\}}) \log{(1/\epsilon)}$ \\
    \hline
    Alg. \ref{alg:DP_OPS_2} for Setting \ref{setting_1} - \ref{setting_3} & $\mathcal{O}(n)$ & $\mathcal{O}(n)$ \\
    \hline
\end{tabular}
\caption{Complexity for generic LP solver and Alg. \ref{alg:DP_OPS_2} ($\tau$, $p$, and $C$ are parameters for the threshold in TPMDP as given in Settings~\ref{setting_1}-\ref{setting_3}. $\epsilon$ is the approximation parameter for LP~\cite{lee2019solving}).}\label{tab:complexity}
%\end{center}
}
\end{table}

\hide{
\textbf{Practical efficiency.} 
We implement Alg. \ref{alg:DP_OPS_2} and compare its efficiency with one of the most efficient LP solvers --- Gurobi~\cite{gurobi}. 
Fig. \ref{fig:eff_a} illustrates the space cost of Grurobi and our algorithm, for variable $n$.
The space requirement of Alg. \ref{alg:DP_OPS_2} is constant with respect to $n$ and clearly smaller than that for Gurobi when $n\geq 15$. 
For Gurobi, in Setting \ref{setting_1} the space cost increases polynomially with $n$;
in Setting \ref{setting_2}, the size of the MPS file increases exponentially with $n$. 
Figs. \ref{fig:eff_b} \& \ref{fig:eff_c} depict the execution time of Gurobi and Alg. \ref{alg:DP_OPS_2} changing with $n$ ($p$ is fixed). 
In Fig. \ref{fig:eff_b}, when $n\leq 12$, the execution time for Gurobi and Alg. \ref{alg:DP_OPS_2} is less than $1$ms.
When $n$ is getting larger, the execution time of Gurobi in Settings \ref{setting_1} \& \ref{setting_2} increases sharply (even exponentially for Setting \ref{setting_2}) while the execution time of Alg. \ref{alg:DP_OPS_2} increases linearly (also presented in Fig. \ref{fig:eff_c}). 
%Actually in Fig. \ref{fig:eff_c}, we find that the execution time of Alg. \ref{alg:DP_OPS_2} for Setting \ref{setting_1} and Setting \ref{setting_2} increases linearly in $n$.
}


==> related.tex <==
In this section, we review previous works related to privacy-preserving collaborative computation and introduce some important definitions and notations that will be used in the following sections.

%In Table \ref{tab:notation} we present the notations that would be used throughout this paper.

%\comment{[notation table]}

%\begin{table}[htbp]\caption{Notations}\label{tab:notation}
%\begin{center}
%\begin{tabular}{r p{7cm} }
%\toprule

%$f(\cdot)$ & A query function \\
%$M(\cdot)$ & A differential privacy mechanism \\
%$U$        & Involved parties in an MPC protocol or multi-party differential %privacy mechanism \\
%$\left|\cdot\right|$ & Absolute value for numbers and length for strings \\

%\bottomrule
%\end{tabular}
%\end{center}
%\label{tab:Notations}
%\end{table}

\subsection{Secure Multi-party Computation}

%Secure multi-party computation (MPC) is a cryptographic tool that enables several parties to collaboratively compute a function while keeping their inputs secret. Formally, with an MPC protocol, a set of parties, $U=\{u_1,u_2,\hdots,u_n\}$, can collaboratively compute a function $f(x_1,x_2,\hdots,x_n)$ where $x_i$ is $u_i$'s input, while the MPC protocol guarantees that if an adversary corrupts a set of parties with arbitrary or restricted size, he can learn nothing other than the output and the input of the corrupted parties. There are two types of MPC protocols. One is information-theoretically secure MPC which is secure against computationally unconstrained adversaries, the other is computationally secure MPC which is secure against poly-time adversaries~\cite{cramer2012secure}.

Secure multi-party computation (MPC) is a cryptographic tool proposed to enable multiple parties to collaboratively compute a function while keeping their inputs secret.
MPC has been extensively studied with the goal of constructing MPC protocols for computing any desired functionality ~\cite{yao1986generate, ben1988completeness,goldreich2009foundations}.
Recently, many works apply MPC protocols to design privacy preserving computation systems, e.g., ridge regression system~\cite{nikolaenko2013privacy}, logistic regression systems~\cite{wu2013privacy} and deep learning systems~\cite{gilad2016cryptonets, jiang2018secure, mohassel2017secureml}.
Meanwhile， many efforts have been devoted to reducing the coputation and communication cost of MPC protocols \cite{ishai2003extending, demmler2015aby}.
%In 1986, Yao.~\cite{yao1986generate} constructs an MPC protocol based on cryptographic tools, namely Garbled Circuits. There is another way to construct MPC protocol based on secret sharing, e.g., \comment{BGW} protocols~\cite{ben1988completeness}. MPC is very powerful, as theoretically, there exist models in which one can construct MPC protocols for computing any desired functionality~\cite{goldreich2009foundations}. Many works apply MPC protocols to design privacy preserving computation systems. In 2013, Nicokaenko et al.~\cite{nikolaenko2013privacy} propose a privacy preserving ridge regression system based on linear homomorphic encryption and Garbled Circuits. Additionally, other approaches include privacy preserving logistic regression systems~\cite{wu2013privacy} and deep learning systems~\cite{gilad2016cryptonets, jiang2018secure} based on homomorphic encryption and Garbled Circuits. In 2017, Mohassel et al.~\cite{mohassel2017secureml} propose SecureML, a privacy preserving machine learning system based on secret sharing, which can accelerate online computation through pre-computation. 
%One drawback of MPC is that the computation and communication complexity of MPC protocols are comparably high, especially those designed for complex computations with large number of parties. Over the years, many works are devoted to improving the performance of MPC protocols. Such works include~\cite{ishai2003extending, demmler2015aby}.
One drawback of MPC is that disclosing the exact function output might leak a party's private input, depending on the background knowledge of the adversary, especially when some parties collude.   

\comment{Problem Setting.} In this work, we consider multi-party collaborative computation of deterministic functions in a semi-honest setting, which means all parties follow the computation protocol honestly but may be curious about other parties' inputs. We assume that the communication channel between each pair of parties is secure. A coalition of adversarial parties can collude and try to recover other parties' private inputs. 

%Now we present the formal definitions of MPC. Here we only care about the security in a semi-honest setting which means all the parties would do the computations honestly but may be curious about other parties' privacy. Also, we consider the communication channel between each pair of parties is private, i.e., an adversary cannot eavesdrop on the conversations between any pair of parties. Thus in this setting, all the adversary can do is to try to collude a set of parties and then try to reconstruct other parties' private information of the other parties. Finally, we only focus on deterministic $f$ in this paper.

Before giving the formal definition of information-theoretically secure MPC in a semi-honest setting, we will first present some important definitions related to MPC.

\begin{definition}[Probability Ensemble~\cite{goldreich2009foundations}]
    Let $I$ be a countable set. An ensemble indexed by $I$ is a sequence of random variables indexed by $I$. Namely, any $X = \{X_i\}_{i\in I}$, where $X_i$ is a random variable, is an ensemble indexed by $I$.
\end{definition}

In this work, we use a set of binary strings $S$ as the index set. Moreover, an ensemble in the form $X = \{X_w\}_{w\in S}$ has each $X_w$ ranging over strings of length $poly(|w|)$ where $|w|$ denotes the binary length of $w$. In multi-party computation, $w$ can be the input of a multi-party computation protocol.

\begin{definition}[Indistinguishability by Polynomial-Sized Circuits~\cite{goldreich2009foundations}]\label{def:poly_ind}
    Two ensembles $X\triangleq \{X_w\}_{w\in S}$ and $Y\triangleq \{Y_w\}_{w\in S}$ are indistinguishable by polynomial-sized circuits, denoted by $X\overset{c}\equiv Y$, if for every family $\{C_n\}_{n\in \mathbb{N}}$ of polynomial-size circuits, every positive polynomial $p(\cdot)$ and all sufficiently long $w$'s,
    \begin{equation}
        \left| \Pr[C_{|w|}(X_{w}) = 1] - \Pr[C_{|w|}(Y_w) = 1] \right| < \frac{1}{p(|w|)}.
    \end{equation}
\end{definition}

We often say computational indistinguishability instead of indistinguishability in polynomial-sized circuits.

\begin{definition}[Statistical Indistinguishability~\cite{goldreich2009foundations}]\label{def:s_ind}
    Two ensembles $X\triangleq \{X_w\}_{w\in S}$ and $Y\triangleq \{Y_w\}_{w\in S}$ are statistically indistinguishable, denoted by $X\overset{s}\equiv Y$, if for every positive polynomial $p(\cdot)$ and all sufficiently long $w$'s,
    \begin{equation}\label{eq:s_ind}
        \Sigma_{\alpha\in \{0,1\}^*} \left| \Pr[X_w =\alpha] - \Pr[Y_w =\alpha] \right| < \frac{1}{p(|w|)}.
    \end{equation}
\end{definition}

%%%%%%%%%%%%%%%%%%%
%An alternative definition of statistical indistinguishability can be derived from the statistical distance of $\Pr[X_w]$ and $\Pr[Y_w]$ which is defined as $\frac{1}{2} (\Sigma_{\alpha\in \{0,1\}^*} \left| \Pr[X_w =\alpha] - \Pr[Y_w =\alpha] \right|$), which is just half of the left-hand side of \eqref{eq:s_ind}.

\begin{definition}[Perfect Indistinguishability~\cite{goldreich2009foundations}]\label{def:perf_ind}
    Two ensembles $X\triangleq \{X_w\}_{w\in S}$ and $Y\triangleq \{Y_w\}_{w\in S}$ are perfectly indistinguishable, denoted by $X\overset{perf}\equiv Y$, if for every $w$,
    \begin{equation}
        \Sigma_{\alpha\in \{0,1\}^*} \left| \Pr[X_w =\alpha] - \Pr[Y_w =\alpha] \right| = 0.
    \end{equation}
\end{definition}

Computational indistinguishability, statistical indistinguishability and perfect indistinguishability are all equivalence relations (reflexive, transitive and symmetric) \cite{lindell2017tutorials, cramer2012secure}. Perfect indistinguishability implies statistical indistinguishability, but not vice versa \cite{meyer1994constructive}. Similarly, statistical indistinguishability implies computational indistinguishability, but not vice versa. 

\begin{definition}[Adversary Structure]
    The adversary structure $\mathcal{A}$ is a family of subsets of the set of parties $U=\{u_1,\hdots,u_n\}$.
\end{definition}

Intuitively, each element in the adversary structure is a subset of parties that the adversary can possibly corrupt. \comment{In this work, we use $\mathcal{A}$ to refer to an adversary structure of all the subsets of $U=\{u_1,\hdots,u_n\}$ by default, i.e., $\mathcal{A} = 2^U$. By slight abuse of notation, we also use $\mathcal{A}$ to refer to the sets of elements in $\mathcal{A}$ corresponding to $U$.}


Subsequently, we provide the definitions of the privacy of MPC in the computational sense and the information-theoretic sense respectively. For convenience, we assume that all the potential inputs of a multi-party computation protocol have the same length, which can be achieved by adequate padding~\cite{goldreich2009foundations}. Then, it is also a natural convention that the function $f$ computed in a multi-party computation protocol is computable in time polynomial in the length of the inputs. Finally, the security is measured in terms of the length of the inputs, i.e., the indistinguishability is measured with respect to the input of the multi-party computation protocol. An alternative way of specifying the aforementioned three conventions is to explicitly specify a security parameter, denoted by $\kappa$, while all the input strings have length $\kappa$, $f(\cdot)$ is computable in polynomial time in $\kappa$. 

%Now, we give the formal definition of the privacy of $n$-party protocols in semi-honest settings with respect to deterministic functions.

We first introduce the security definition of MPC in a high level. For a $n$-ary deterministic function $f:\ (\{0,1\}^{*})^n\rightarrow (\{0,1\}^{*})^n$, where $f_i(x_1,x_2,\hdots,x_n)$ denotes the $i$-th element of $f(x_1,x_2,\hdots,x_n)$, we let $f_A(x_1,\hdots,x_n)$ denotes $(f_{i_1}(x_1,\hdots,x_n),\hdots,f_{i_{t'}}(x_1,\hdots,x_n))$ where $A=\{i_1,\hdots,i_{t'}\} \in \mathcal{A}$. The \textbf{view} of the party $u_j,\, j\in \{1,2,\hdots,n\}$ during an execution of $\Pi$ on $\bar{x} = (x_1,x_2,\hdots,x_n) \in (\{0,1\}^{*})^n$, denoted by $View_{j}^{\Pi}(\bar{x})$, is $(x_j,r_j,m_1,\hdots,m_N)$, where $x_j$ represents the input of $u_j$, $r_j$ represents $u_j$'s internal coin toss, and $m_i$ represents the $i$-th message it receives during the execution for $i\in \{1,\hdots,N\}$. The \textbf{output} of $u_i$ after an execution of $\Pi$ on $\bar{x}$, denoted by $Output_i^{\Pi}(\bar{x})$, is implicit in $u_i$'s own view of the execution, and $Output^{\Pi}=(Output_1^{\Pi}(\bar{x}),Output_2^{\Pi}(\bar{x}),\hdots,Output_n^{\Pi}(\bar{x}))$. For $A=\{i_1,\hdots,i_{t'}\} \in \mathcal{A}$, we let $View_A^\Pi(\bar{x}) \triangleq (A, View_{i_1}^\Pi (\bar{x}),\hdots,View_{i_{t'}}^\Pi (\bar{x}))$. Recall that what MPC guarantee is that each party or each size-constrained adversary set can learn nothing but the information that can be inferred from the output result. Thus, we say a protocol privately computes $f$ if whatever can be obtained from $A$'s view i.e., $View_A^\Pi(\bar{x})$ could be essentially obtained from the inputs and outputs available to $A$ for $A\in \mathcal{A}$. Now, we are ready to give the formal definition of computationally secure MPC.

\begin{definition}[privacy of $n$-party protocols for deterministic functions in semi-honest settings~\cite{goldreich2009foundations}]\label{def:c_MPC}
    We say that \textbf{$\Pi$ privately computes} $f$ if there exists a probabilistic polynomial-time algorithm, denoted by $\mathcal{S}$, such that for every $A=\{i_1,\hdots,i_{t'}\} \in \mathcal{A}$, it holds that 
    \begin{equation}\label{eq:c_deter_MPC}
        \begin{aligned}
            \{\mathcal{S}(A,(x_{i_1},\hdots,x_{i_{t'}}), & f_A(\bar{x}))\}_{\bar{x}\in (\{0,1\}^{*})^n} \overset{c}\equiv \\
            & \{View_A^\Pi (\bar{x})\}_{\bar{x}\in (\{0,1\}^{*})^n}.
        \end{aligned}
    \end{equation}
\end{definition}

In information-theoretically secure MPC, as posed in~\cite{goldreich2009foundations}, security holds only in case the honest parties are in a strict majority. So we usually consider an adversary structure in which the cardinality of any adversary set is constrained by a predefined threshold $t$, i.e., $ \left| A \right| \leq t $ for all $A\in \mathcal{A}$. Also we believe that it is indeed a meaningful assumption as in many real-world applications, it is hard to collude large number of parties. Furthermore, we denote by $\mathcal{A}_t$ the adversary structure corresponding to such $t$-threshold security model, i.e.,
\begin{equation}\label{eq:t_AS}
    \mathcal{A}_t=\{A\in 2^\emph{U} | \left|A\right| \leq t\}.
\end{equation}


\begin{definition}[$t$-privacy of $n$-party protocols for deterministic functions in semi-honest settings~\cite{goldreich2009foundations}]\label{def:t_MPC}
    We say that \textbf{$\Pi$ $t$-privately computes} $f$ if there exists a probabilistic polynomial-time algorithm, denoted by $\mathcal{S}$, such that for every $A=\{i_1,\hdots,i_{t'}\} \in \mathcal{A}_t$, it holds that 
    \begin{equation}\label{eq:deter_MPC}
        \begin{aligned}
            \{\mathcal{S}(A,(x_{i_1},\hdots,x_{i_{t'}}), & f_A(\bar{x}))\}_{\bar{x}\in (\{0,1\}^{*})^n} \overset{s}\equiv\\
            &\{View_A^\Pi (\bar{x})\}_{\bar{x}\in (\{0,1\}^{*})^n}.
        \end{aligned}
    \end{equation} 
    
    In case the ensembles in \eqref{eq:deter_MPC} are \textbf{perfectly indistinguishable}, we say that \textbf{the emulation is perfect}.
\end{definition}

An MPC protocol which can $t$-privately computes a class of functions with $n$ parties is called a $(t,n)$-threshold MPC protocol. 

Although in the standard definition of MPC, an MPC protocol is designed to handle the inputs in $(\{0,1\}^{*})^n$, one can also design an MPC protocol which can process non-negative finite-precision numbers by some encoding techniques and negative numbers can be represented using the standard two’s complement representation~\cite{nikolaenko2013privacy}. 



\subsection{Differential Privacy}
We begin by presenting the definition of differential privacy, followed by the introduction of an important class of differential privacy mechanisms, i.e., Gaussian output perturbation mechanisms. In the last part of this subsection, we present the composition properties of differential privacy, which are useful to design a sophisticated differential privacy mechanism from simpler ones.

%The concept of Differential Privacy is introduced by Dwork et al.~\cite{cynthia2006differential}, which gives a metric to evaluate the privacy loss with respect to an individual in a randomization mechanism. 

In differential privacy, we are interested in measuring privacy guarantees provided by a randomized mechanism $M$ with domain $2^\mathcal{X}$, where $\mathcal{X}$ is a finite set. For $x,y\in 2^\mathcal{X}$, when we say that $x$ and $y$ are neighbouring inputs, written as $x\simeq y$, we mean they are identical or one can be obtained from the other by replacing a single element. Intuitively, differential privacy requires that when changing the input from $x$ to $y$ where $x\simeq y$, the output distribution of $M$ would not change drastically. Formally, the definition of differential privacy is given in Definition \ref{def:DP}.

\begin{definition}[Differential Privacy]~\cite{dwork2014algorithmic}\label{def:DP}
    For $\epsilon\geq 0$, $\delta \in [0,1]$, a randomized algorithm $M$ with domain $2^\mathcal{X}$ is $(\epsilon, \delta)$-differentially private if for all $S \subset Range(M)$ and for all $x, y \in 2^\mathcal{X}$ such that $x\simeq y$: 
    \begin{equation}\label{eq:DP}
        \Pr[M(x) \in S] \leq \exp(\epsilon) \Pr[M(y) \in S] + \delta.
    \end{equation}
\end{definition}

An important class of differential privacy mechanisms involves output perturbation, which achieves differential privacy by adding output-independent noise to the original output of a query, i.e., given a query function $f:\ 2^\mathcal{X}\rightarrow \mathbb{R}^d$, an output perturbation mechanism $M$ is like
$$M(x)=f(x)+X,$$
where $X$ is a noise value independent of $x$. Such output perturbation schemes include Laplace Mechanism~\cite{dwork2014algorithmic}, Gaussian Mechanism~\cite{dwork2014algorithmic} and Staircase Mechanism~\cite{geng2014optimal}. 

Our work in this paper is related to Gaussian Mechanism which is an output perturbation mechanism with $X\sim \mathcal{N}(0,\sigma^2 I)$ where $I$ is the $d$-dimensional identity matrix (also referred as a Gaussian output perturbation mechanism). \cite{dwork2014algorithmic} proposes the theorem of Gaussian Mechanism which gives a way to select the standard deviation of the noise, i.e., $\sigma$ with respect to $f$ such that the resulting output perturbation mechanism is $(\epsilon,\delta)$--differentially private. However, It was shown in~\cite{balle2018improving} that the classical Gaussian Mechanism in \cite{dwork2014algorithmic} is not tight, which means that given $\Delta_2 f$, $\epsilon$ and $\delta$, one can usually obtain an $(\epsilon,\delta)$--differential private Gaussian output perturbation mechanism with smaller $\sigma$ than specified in the classical Gaussian Mechanism. To overcome this limitation, they provide an analytic way to select $\sigma$ such that the resulting Gaussian output perturbation mechanism is tight for $(\epsilon,\delta)$--differential privacy. The resulting mechanism is called Analytical Gaussian Mechanism.

Before presenting the theorem of Analytical Gaussian mechanism, we will first introduce $l_2$--sensitivity, which is an important notion in Differential Privacy.

\begin{definition}[$l_2$-sensitivity]
The $l_2$-sensitivity of a function $f:\ 2^\mathcal{X}\rightarrow \mathbb{R}^d$ is:
\begin{equation}
\Delta_2 f = \mathop{\max}\limits_{\mathop{x,y\in{2^\mathcal{X}}}\limits_{x\simeq y}}\left\|f(x)-f(y)\right\|_2.
\end{equation}
\end{definition}

\begin{theorem}[Analytical Gaussian Mechanism]~\cite{balle2018improving}\label{thm:AGM}
    For $\epsilon \geq 0$ and $\delta\in [0,1]$, the Gaussian output perturbation mechanism with $X\sim \mathcal{N}(0,\sigma^2 I)$ is $(\epsilon,\delta)$--differential private if and only if
    \begin{equation}\label{eq:AGM}
        \Phi \left( \frac{\Delta_2 f}{2\sigma}-\frac{\epsilon \sigma}{\Delta_2 f} \right) - \exp{(\epsilon)} \Phi \left( -\frac{\Delta_2 f}{2\sigma}-\frac{\epsilon \sigma}{\Delta_2 f} \right) \leq \delta,
    \end{equation}
    where $\Phi(\cdot)$ is the cumulative density function of $\mathcal{N}(0,1)$.
\end{theorem}

Given $\epsilon\geq 0$, $\delta \in [0,1]$ and $\Delta_2 f$, one can solve~\eqref{eq:AGM} for $\sigma_{(\epsilon,\delta, \Delta_2 f)}$ with a very efficient numerical computation algorithm presented in~\cite{balle2018improving} such that \eqref{eq:AGM} holds if and only if $\sigma \geq \sigma_{(\epsilon,\delta, \Delta_2 f)}$. The formal definition of $\sigma_{(\epsilon,\delta, \Delta_2 f)}$ is presented in Definition \ref{def:sigma_Gamma}.

%As mentioned in~\cite{balle2018improving}, $\sigma_{(\epsilon,\delta, \Delta_2 f)}$ is exactly the lower bound of the standard deviation of Gaussian output perturbation mechanisms for $f(\cdot)$ which satisfy $(\epsilon,\delta)$--differential privacy, i.e., a Gaussian output perturbation mechanism for $f(\cdot)$ with $X\sim \mathcal{N}(0,\sigma^2 I)$ is $(\epsilon,\delta)$--differentially private if and only if $\sigma \geq \sigma_{(\epsilon,\delta, \Delta_2 f)}$. 

\begin{definition}\label{def:sigma_Gamma}
    Given the tuple $\Gamma\triangleq (\epsilon, \delta, \Delta_2 f)$ ,$\sigma_{(\epsilon,\delta, \Delta_2 f)}$ is the lower bound of $\sigma$ such that the Gaussian mechanism with the additive noise $X\sim \mathcal{N}(0, \sigma^2)$ is $(\epsilon, \delta)$--DP.
\end{definition}

It holds that \comment{$\sigma_{(\epsilon,\delta, \Delta_2 f)}$ is continuous with respect to $\epsilon$, $\delta$, $\Delta_2 f$. Furthermore, it decreases monotonically with $\epsilon$, $\delta$ and increases monotonically with $\Delta_2 f$}. 
%For simplification, we denote $(\epsilon,\delta, \Delta_2 f)$ by $\Gamma$ and then we use $\sigma_{\Gamma}$ to refer to $\sigma_{(\epsilon,\delta, \Delta_2 f)}$ in the rest of this paper.
Now, we introduce the composition theorem as well as the advanced one for differential privacy.

\begin{theorem}[Composition Theorem]\label{thm:comp_thm}~\cite{dwork2014algorithmic}
    Let $M_i: 2^\mathcal{X} \rightarrow \mathcal{R}_i$ be an $(\epsilon_i,\delta_i)$--differentially private algorithm for $i\in \{1,2,\hdots,k\}$. Then if $M_{[k]}: 2^\mathcal{X} \rightarrow \bigotimes_{i=1}^k \mathcal{R}_i$ is defined as $M_{[k]}(x) = (M_1(x),\hdots,M_k(x))$, then $M_{[k]}$ is $(\Sigma_{i=1}^k \epsilon_i, \Sigma_{i=1}^k \delta_i)$--differential private.
\end{theorem}

\begin{theorem}[Advanced Composition]\label{thm:A_comp}~\cite{dwork2014algorithmic}
    For all $\epsilon,\delta,\delta^{'} \geq 0$, the class of $(\epsilon,\delta)$--differential private mechanisms satisfies $(\epsilon^{'},k\delta+\delta^{'})$--differential privacy under $k$--fold adaptive composition for:%
    \begin{equation}
        \epsilon^{'} = \sqrt{2k\ln{1/\delta^{'}}}\epsilon + k\epsilon(\exp{(\epsilon)}-1).
    \end{equation}
\end{theorem}



Notice that the original definition of differential privacy considers adversaries with unbounded computational power. In 2009, Mironov et al.~\cite{mironov2009computational} present the definition of computational differential privacy, which is a relaxation of the original definition. The definition of computational differential privacy requires privacy guarantees to hold only against computationally bounded (polynomial-time) adversaries. In 2015, Jorgensen et al.~\cite{jorgensen2015conservative} generalize the idea of differential privacy by introducing the concept of personalized differential privacy. As differential privacy provides a theoretical guarantee for protecting the private information contained in the output, many works about privacy preserving computation systems choose differential privacy mechanisms as components in their designs~\cite{abadi2016deep, iyengar2019towards, mckenna2019graphical, jagielski2018differentially}. 

The drawback of differential privacy is that the utility of a differentially private mechanism would deteriorate due to the perturbation of the original result. There are also many works devoted to finding the optimal differentially private mechanism with respect to the utility. For example, Geng et al. propose a family of mechanisms and prove their optimality with respect to monotone utility functions for different query functions and different privacy requirements. Those mechanisms include staircase mechanism for $\epsilon$-differential privacy~\cite{geng2014optimal}, multi-dimensional staircase mechanism for $\epsilon$-differential privacy with multi-dimensional query functions~\cite{geng2013optimal}. They also propose an asymptotically optimal mechanism for $(\epsilon, \delta)$--differential privacy called the truncated Laplacian mechanism~\cite{geng2015optimal}. Balle et al.~\cite{balle2018improving} proposes the optimal Gaussian output perturbation mechanisms, namely the Analytical Gaussian mechanism.


\subsection{Multi-party Differential Privacy}



Differential privacy can be extended to accommodate the settings of multi-party computations. In 2006, Dwork et al.~\cite{dwork2006our} propose a securely distributed noise generation protocol called \emph{Our Data, Ourselves} (ODO) against malicious adversaries. ODO facilitates the construction of a multi-party differentially private mechanism as we can construct the mechanism by designing a SFE protocol for computing the query function perturbated by additive noises generated by ODO. In 2011, Beimel et al.~\cite{nissim2011distributed} give a formal definition for threshold personalized multi-party differential privacy (TPMDP) against semi-honest adversaries with respect to the information theoretic setting as well as the computationally bounded setting and propose several example multi-party differentially private mechanisms for computing the binary sum function. They present two methods to construct multi-party differentially private mechanisms to compute binary sum function, one is combining SFE and differentially private mechanisms, the other one is purely based on randomized response, which is a well-known mechanism in local differential privacy. As the methodology combining SFE and differential privacy is usually superior in accuracy, many works in privacy preserving computation systems with strong accuracy requirements are constructed in this way. For example, Goryczka et al.~\cite{goryczka2013secure} construct a multi-party protocol to compute sum query functions over several parties' inputs based on MPC and differential privacy. Similarly, Papadimitriou et al.~\cite{papadimitriou2017dstress} combine secret sharing, homomorphic encryption and differential privacy to construct a privacy-preserving large-scale graph analysis system. Acar et al.~\cite{acar2017achieving} also present a privacy-preserving distributed linear regression system with the similar methodology.

An important subclass of multi-party differential privacy is local differential privacy (LDP)~\cite{warner1965randomized}, in which each party with inputs only communicates with a special third party called the curator who could be one of the parties providing inputs. The curator would complete the computation of a given function with inputs from all involved parties. Local differential privacy demands that each party's input should remain differentially private even if the curator is semi-honest.~\cite{nissim2011distributed} compares LDP mechanisms and the mechanisms combining SFE and differential privacy. It shows that LDP mechanisms may be more efficient but would introduce more noise or perturbation.~\cite{kairouz2015secure} further proves that the non-interactive randomized response which is one of the simplest LDP mechanisms, is optimal in LDP when each party holds a single bit of information. Specially, the setting they consider is slightly different from the standard LDP setting where each party could hold a different privacy requirement and a different function to compute, which is similar as the setting we consider in this paper. Actually, it is not difficult to see that the standard LDP setting is just a special case of the setting they consider. As LDP is superior in efficiency especially when the computation involving a large number of parties, many works try to construct efficient differentially private distributed computation systems based on LDP~\cite{polatidis2017privacy, ye2019privkv, wang2019collecting}. Also, there exist many works trying to improve the accuracy of LDP mechanisms ~\cite{kairouz2014extremal, duchi2018minimax}. Specially,~\cite{cheu2019distributed} proposes a shuffled model which lies between the local model considered in LDP and the central model where all the data are owned by a single server. With the help of an anonymous channel called a shuffler, the accuracy of the shuffled model would be strictly between the local and the central one.

%\section{Preliminary}\label{sec:prel}



%\subsection{Differential privacy}

%We begin by presenting the definition of differential privacy, followed by the introduction of an important class of differential privacy mechanisms, i.e., Gaussian output perturbation mechanisms. In the last part of this subsection, we present the composition properties of differential privacy, which are useful to design a sophisticated differential privacy mechanism from simpler ones.



%\begin{theorem}[Post-Processing]
    
%\end{theorem}

%\subsection{Secure multi-party computation}
%Secure multi-party computation (MPC) is a cryptographic tool that enables several parties to collaboratively compute a function while keeping their inputs secret. Formally, with an MPC protocol, a set of parties, $U=\{u_1,u_2,\hdots,u_n\}$, can collaboratively compute a function $f(x_1,x_2,\hdots,x_n)$ where $x_i$ is $u_i$'s input, while the MPC protocol guarantees that if an adversary corrupts a set of parties with arbitrary or restricted size, he can learn nothing other than the output and the input of the corrupted parties. There are two types of MPC protocols. One is information-theoretically secure MPC which is secure against computationally unconstrained adversaries, the other is computationally secure MPC which is secure against poly-time adversaries~\cite{cramer2012secure}. 

%In this paper, we focus on both computationally and information-theoretically secure MPC protocols. 

%As mentioned before, here we only care about the security in a semi-honest setting which means all the parties would do the computations honestly but may be curious about other parties' privacy. Also, we consider the communication channel between each pair of parties is private, i.e., an adversary cannot eavesdrop on the conversations between any pair of parties. Thus in this setting, all the adversary can do is to try to collude a set of parties $A$ and then try to reconstruct other parties' private information of the other parties in $\bar{A}$. 

%Before giving the formal definition of information-theoretically secure MPC in semi-honest settings, we will first present some important definitions related to MPC.
